Blue quantum emitter in hexagonal boron nitride and carbon chain tetramer: proposition of identification

Single photon emitters in hexagonal boron nitride offer a gateway to the future of quantum technologies, yet their identification remains challenging and subject to ongoing debate. We demonstrate through ab initio calculations that the optical properties of a carbon chain tetramer are in excellent agreement with the characteristics of a blue quantum emitter in hexagonal boron nitride emitting at 435 nm. Its calculated zero-phonon line energy (2.77 eV) and radiative lifetime (1.6 ns) perfectly align with experimental observations. The relatively weak electron--phonon coupling (Huang-Rhys factor of 1.5) indicates intense emission at the zero-phonon line. Despite the absence of an inversion center in the carbon tetramer, we demonstrate that it exhibits a negligible linear Stark effect, consistent with experimental findings. Additionally, our hypothesis explains the experimental observation that the formation of blue emitters is only possible in samples containing numerous ultraviolet emitters, which are likely identical to carbon dimers.

==> bib.tex <==
@article{Shevitski,
  title = {Blue-light-emitting color centers in high-quality hexagonal boron nitride},
  author = {Shevitski, Brian and Gilbert, S. Matt and Chen, Christopher T. and Kastl, Christoph and Barnard, Edward S. and Wong, Ed and Ogletree, D. Frank and Watanabe, Kenji and Taniguchi, Takashi and Zettl, Alex and Aloni, Shaul},
  journal = {Phys. Rev. B},
  volume = {100},
  issue = {15},
  pages = {155419},
  numpages = {9},
  year = {2019},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.100.155419},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.100.155419}
}

@article{Zhigulin1,
doi = {10.1088/2633-4356/acb87f},
url = {https://dx.doi.org/10.1088/2633-4356/acb87f},
year = {2023},
month = {mar},
publisher = {IOP Publishing},
volume = {3},
number = {1},
pages = {015002},
author = {Ivan Zhigulin and Karin Yamamura and Viktor Ivády and Angus Gale and Jake Horder and Charlene J Lobo and Mehran Kianinia and Milos Toth and Igor Aharonovich},
title = {Photophysics of blue quantum emitters in hexagonal boron nitride},
journal = {Materials for Quantum Technology }
}

@article{Zhigulin2,
  title = {Stark Effect of Blue Quantum Emitters in Hexagonal Boron Nitride},
  author = {Zhigulin, Ivan and Horder, Jake and Iv\'ady, Viktor and White, Simon J.U. and Gale, Angus and Li, Chi and Lobo, Charlene J. and Toth, Milos and Aharonovich, Igor and Kianinia, Mehran},
  journal = {Phys. Rev. Appl.},
  volume = {19},
  issue = {4},
  pages = {044011},
  numpages = {7},
  year = {2023},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevApplied.19.044011},
  url = {https://link.aps.org/doi/10.1103/PhysRevApplied.19.044011}
}

@article{Chen_annealing,
    author = {Chen, Yongliang and Gale, Angus and Yamamura, Karin and Horder, Jake and Condos, Alexander and Watanabe, Kenji and Taniguchi, Takashi and Toth, Milos and Aharonovich, Igor},
    title = "{Annealing of blue quantum emitters in carbon-doped hexagonal boron nitride}",
    journal = {Applied Physics Letters},
    volume = {123},
    number = {4},
    pages = {041902},
    year = {2023},
    month = {07},
    issn = {0003-6951},
    doi = {10.1063/5.0155311},
    url = {https://doi.org/10.1063/5.0155311},
    eprint = {https://pubs.aip.org/aip/apl/article-pdf/doi/10.1063/5.0155311/18056302/041902\_1\_5.0155311.pdf}
}

@Article{Ganyecz,
author ="Ganyecz, {\'A}d{\'a}m and Babar, Rohit and Benedek, Zsolt and Aharonovich, Igor and Barcza, Gergely and Ivády, Viktor",
title  ="First-principles theory of the nitrogen interstitial in hBN: a plausible model for the blue emitter",
journal  ="Nanoscale",
year  ="2024",
volume  ="16",
issue  ="8",
pages  ="4125-4139",
publisher  ="The Royal Society of Chemistry",
doi  ="10.1039/D3NR05811E",
url  ="http://dx.doi.org/10.1039/D3NR05811E"
}

@article{Kresse_vasp,
  title = {Efficient iterative schemes for ab initio total-energy calculations using a plane-wave basis set},
  author = {Kresse, G. and Furthm\"uller, J.},
  journal = {Phys. Rev. B},
  volume = {54},
  issue = {16},
  pages = {11169--11186},
  numpages = {0},
  year = {1996},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.54.11169},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.54.11169}
}

@article{Blochl,
  title = {Projector augmented-wave method},
  author = {Bl\"ochl, P. E.},
  journal = {Phys. Rev. B},
  volume = {50},
  issue = {24},
  pages = {17953--17979},
  numpages = {0},
  year = {1994},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.50.17953},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.50.17953}
}

@article{Heyd,
    author = {Heyd, Jochen and Scuseria, Gustavo E. and Ernzerhof, Matthias},
    title = "{Hybrid functionals based on a screened Coulomb potential}",
    journal = {The Journal of Chemical Physics},
    volume = {118},
    number = {18},
    pages = {8207-8215},
    year = {2003},
    month = {05},
    issn = {0021-9606},
    doi = {10.1063/1.1564060},
    url = {https://doi.org/10.1063/1.1564060},
    eprint = {https://pubs.aip.org/aip/jcp/article-pdf/118/18/8207/19093575/8207\_1\_online.pdf}
}

@article{Tomaszkiewicz,
    author={Tomaszkiewicz, Iwona},
    title={The Enthalpy of Formation of Hexagonal Boron Nitride},
    journal={Pol. J. Chem.},
    volume={76},
    number={6},
    pages={891-899},
    year={2002}
}

@article{Sun_SCAN,
  title = {Strongly Constrained and Appropriately Normed Semilocal Density Functional},
  author = {Sun, Jianwei and Ruzsinszky, Adrienn and Perdew, John P.},
  journal = {Phys. Rev. Lett.},
  volume = {115},
  issue = {3},
  pages = {036402},
  numpages = {6},
  year = {2015},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.115.036402},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.115.036402}
}

@article{Furness_r2SCAN,
    author = {Furness, James W. and Kaplan, Aaron D. and Ning, Jinliang and Perdew, John P. and Sun, Jianwei},
    title = {Accurate and Numerically Efficient r2SCAN Meta-Generalized Gradient Approximation},
    journal = {The Journal of Physical Chemistry Letters},
    volume = {11},
    number = {19},
    pages = {8208-8215},
    year = {2020},
    doi = {10.1021/acs.jpclett.0c02405},
    note ={PMID: 32876454},
    URL = {https://doi.org/10.1021/acs.jpclett.0c02405},
    eprint = {https://doi.org/10.1021/acs.jpclett.0c02405}
}

@article{Maciaszek_JCP,
    author = {Maciaszek, Marek and Žalandauskas, Vytautas and Silkinis, Rokas and Alkauskas, Audrius and Razinkovas, Lukas},
    title = "{The application of the SCAN density functional to color centers in diamond}",
    journal = {The Journal of Chemical Physics},
    volume = {159},
    number = {8},
    pages = {084708},
    year = {2023},
    month = {08},
    doi = {10.1063/5.0154319},
    url = {https://doi.org/10.1063/5.0154319},
    eprint = {https://pubs.aip.org/aip/jcp/article-pdf/doi/10.1063/5.0154319/18102318/084708\_1\_5.0154319.pdf},
}

@article{Grimme,
author = {Grimme, Stefan},
title = {Semiempirical GGA-type density functional constructed with a long-range dispersion correction},
journal = {Journal of Computational Chemistry},
volume = {27},
number = {15},
pages = {1787-1799},
keywords = {density functional theory, generalized gradient approximation, van der Waals interactions, thermochemistry},
doi = {https://doi.org/10.1002/jcc.20495},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/jcc.20495},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1002/jcc.20495},
year = {2006}
}

@article{Dion,
  title = {Van der Waals Density Functional for General Geometries},
  author = {Dion, M. and Rydberg, H. and Schr\"oder, E. and Langreth, D. C. and Lundqvist, B. I.},
  journal = {Phys. Rev. Lett.},
  volume = {92},
  issue = {24},
  pages = {246401},
  numpages = {4},
  year = {2004},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.92.246401},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.92.246401}
}

@article{Roman-Perez,
  title = {Efficient Implementation of a van der Waals Density Functional: Application to Double-Wall Carbon Nanotubes},
  author = {Rom\'an-P\'erez, Guillermo and Soler, Jos\'e M.},
  journal = {Phys. Rev. Lett.},
  volume = {103},
  issue = {9},
  pages = {096102},
  numpages = {4},
  year = {2009},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.103.096102},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.103.096102}
}

@article{Klimes,
  title = {Van der Waals density functionals applied to solids},
  author = {Klime\ifmmode \check{s}\else \v{s}\fi{}, Ji\ifmmode \check{r}\else \v{r}\fi{}\'{\i} and Bowler, David R. and Michaelides, Angelos},
  journal = {Phys. Rev. B},
  volume = {83},
  issue = {19},
  pages = {195131},
  numpages = {13},
  year = {2011},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.83.195131},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.83.195131}
}

@article{Peng_rVV10,
  title = {Versatile van der Waals Density Functional Based on a Meta-Generalized Gradient Approximation},
  author = {Peng, Haowei and Yang, Zeng-Hui and Perdew, John P. and Sun, Jianwei},
  journal = {Phys. Rev. X},
  volume = {6},
  issue = {4},
  pages = {041005},
  numpages = {15},
  year = {2016},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevX.6.041005},
  url = {https://link.aps.org/doi/10.1103/PhysRevX.6.041005}
}

@article{Zhang_Northrup,
  title = {Chemical potential dependence of defect formation energies in GaAs: Application to Ga self-diffusion},
  author = {Zhang, S. B. and Northrup, John E.},
  journal = {Phys. Rev. Lett.},
  volume = {67},
  issue = {17},
  pages = {2339--2342},
  numpages = {0},
  year = {1991},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.67.2339},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.67.2339}
}

@article{Freysoldt_RevModPhys,
  title = {First-principles calculations for point defects in solids},
  author = {Freysoldt, Christoph and Grabowski, Blazej and Hickel, Tilmann and Neugebauer, J\"org and Kresse, Georg and Janotti, Anderson and Van de Walle, Chris G.},
  journal = {Rev. Mod. Phys.},
  volume = {86},
  issue = {1},
  pages = {253--305},
  numpages = {53},
  year = {2014},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.86.253},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.86.253}
}

@article{Freysoldt_PRL,
  title = {Fully Ab Initio Finite-Size Corrections for Charged-Defect Supercell Calculations},
  author = {Freysoldt, Christoph and Neugebauer, J\"org and Van de Walle, Chris G.},
  journal = {Phys. Rev. Lett.},
  volume = {102},
  issue = {1},
  pages = {016402},
  numpages = {4},
  year = {2009},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.102.016402},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.102.016402}
}

@article{Maciaszek_PRM,
  title = {Thermodynamics of carbon point defects in hexagonal boron nitride},
  author = {Maciaszek, Marek and Razinkovas, Lukas and Alkauskas, Audrius},
  journal = {Phys. Rev. Mater.},
  volume = {6},
  issue = {1},
  pages = {014005},
  numpages = {13},
  year = {2022},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevMaterials.6.014005},
  url = {https://link.aps.org/doi/10.1103/PhysRevMaterials.6.014005}
}

@article{Weston,
  title = {Native point defects and impurities in hexagonal boron nitride},
  author = {Weston, L. and Wickramaratne, D. and Mackoit, M. and Alkauskas, A. and Van de Walle, C. G.},
  journal = {Phys. Rev. B},
  volume = {97},
  issue = {21},
  pages = {214104},
  numpages = {13},
  year = {2018},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.97.214104},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.97.214104}
}

@article{Gale,
    author = {Gale, Angus and Li, Chi and Chen, Yongliang and Watanabe, Kenji and Taniguchi, Takashi and Aharonovich, Igor and Toth, Milos},
    title = {Site-Specific Fabrication of Blue Quantum Emitters in Hexagonal Boron Nitride},
    journal = {ACS Photonics},
    volume = {9},
    number = {6},
    pages = {2170-2177},
    year = {2022},
    doi = {10.1021/acsphotonics.2c00631},
    URL = {https://doi.org/10.1021/acsphotonics.2c00631},
    eprint = {https://doi.org/10.1021/acsphotonics.2c00631}
}

@article{Mackoit_dimer,
    author = {Mackoit-Sinkevičienė, M. and Maciaszek, M. and Van de Walle, C. G. and Alkauskas, A.},
    title = "{Carbon dimer defect as a source of the 4.1 eV luminescence in hexagonal boron nitride}",
    journal = {Applied Physics Letters},
    volume = {115},
    number = {21},
    pages = {212101},
    year = {2019},
    month = {11},
    issn = {0003-6951},
    doi = {10.1063/1.5124153},
    url = {https://doi.org/10.1063/1.5124153},
    eprint = {https://pubs.aip.org/aip/apl/article-pdf/doi/10.1063/1.5124153/13286483/212101\_1\_online.pdf},
}

@article{Auburger,
  title = {Towards ab initio identification of paramagnetic substitutional carbon defects in hexagonal boron nitride acting as quantum bits},
  author = {Auburger, Philipp and Gali, Adam},
  journal = {Phys. Rev. B},
  volume = {104},
  issue = {7},
  pages = {075410},
  numpages = {12},
  year = {2021},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.104.075410},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.104.075410}
}

@Article{Fournier,
author={Fournier, Clarisse
and Plaud, Alexandre
and Roux, S{\'e}bastien
and Pierret, Aur{\'e}lie
and Rosticher, Michael
and Watanabe, Kenji
and Taniguchi, Takashi
and Buil, St{\'e}phanie
and Qu{\'e}lin, Xavier
and Barjon, Julien
and Hermier, Jean-Pierre
and Delteil, Aymeric},
title={Position-controlled quantum emitters with reproducible emission wavelength in hexagonal boron nitride},
journal={Nature Communications},
year={2021},
month={Jun},
day={18},
volume={12},
number={1},
pages={3779},
issn={2041-1723},
doi={10.1038/s41467-021-24019-6},
url={https://doi.org/10.1038/s41467-021-24019-6}
}

@article{Geick,
  title = {Normal Modes in Hexagonal Boron Nitride},
  author = {Geick, R. and Perry, C. H. and Rupprecht, G.},
  journal = {Phys. Rev.},
  volume = {146},
  issue = {2},
  pages = {543--547},
  numpages = {0},
  year = {1966},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRev.146.543},
  url = {https://link.aps.org/doi/10.1103/PhysRev.146.543}
}

@article{Jones,
  title = {The density functional formalism, its applications and prospects},
  author = {Jones, R. O. and Gunnarsson, O.},
  journal = {Rev. Mod. Phys.},
  volume = {61},
  issue = {3},
  pages = {689--746},
  numpages = {0},
  year = {1989},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.61.689},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.61.689}
}

@article{Alkauskas_PRL,
  title = {First-Principles Calculations of Luminescence Spectrum Line Shapes for Defects in Semiconductors: The Example of GaN and ZnO},
  author = {Alkauskas, Audrius and Lyons, John L. and Steiauf, Daniel and Van de Walle, Chris G.},
  journal = {Phys. Rev. Lett.},
  volume = {109},
  issue = {26},
  pages = {267401},
  numpages = {5},
  year = {2012},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.109.267401},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.109.267401}
}

@Article{Grudinin,
author ="Grudinin, D. V. and Ermolaev, G. A. and Baranov, D. G. and Toksumakov, A. N. and Voronin, K. V. and Slavich, A. S. and Vyshnevyy, A. A. and Mazitov, A. B. and Kruglov, I. A. and Ghazaryan, D. A. and Arsenin, A. V. and Novoselov, K. S. and Volkov, V. S.",
title  ="Hexagonal boron nitride nanophotonics: a record-breaking material for the ultraviolet and visible spectral ranges",
journal  ="Mater. Horiz.",
year  ="2023",
volume  ="10",
issue  ="7",
pages  ="2427-2435",
publisher  ="The Royal Society of Chemistry",
doi  ="10.1039/D3MH00215B",
url  ="http://dx.doi.org/10.1039/D3MH00215B"
}

@article{Lee,
author = {Lee, Seong-Yeon and Jeong, Tae-Young and Jung, Suyong and Yee, Ki-Ju},
title = {Refractive Index Dispersion of Hexagonal Boron Nitride in the Visible and Near-Infrared},
journal = {physica status solidi (b)},
volume = {256},
number = {6},
pages = {1800417},
keywords = {hexagonal boron nitride, refractive index dispersion, single oscillator model},
doi = {https://doi.org/10.1002/pssb.201800417},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/pssb.201800417},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1002/pssb.201800417},
year = {2019}
}

@article{Aharonovich_Nanolett,
author = {Aharonovich, Igor and Tetienne, Jean-Philippe and Toth, Milos},
title = {Quantum Emitters in Hexagonal Boron Nitride},
journal = {Nano Letters},
volume = {22},
number = {23},
pages = {9227-9235},
year = {2022},
doi = {10.1021/acs.nanolett.2c03743},
note ={PMID: 36413674},
URL = {https://doi.org/10.1021/acs.nanolett.2c03743},
eprint = {https://doi.org/10.1021/acs.nanolett.2c03743}
}

@article{Caldwell,
author={Caldwell, Joshua D.
and Aharonovich, Igor
and Cassabois, Guillaume
and Edgar, James H.
and Gil, Bernard
and Basov, D. N.},
title={Photonics with hexagonal boron nitride},
journal={Nature Reviews Materials},
year={2019},
month={Aug},
day={01},
volume={4},
number={8},
pages={552-567},
issn={2058-8437},
doi={10.1038/s41578-019-0124-1},
url={https://doi.org/10.1038/s41578-019-0124-1}
}

@article{Tran,
author={Tran, Toan Trong
and Bray, Kerem
and Ford, Michael J.
and Toth, Milos
and Aharonovich, Igor},
title={Quantum emission from hexagonal boron nitride monolayers},
journal={Nature Nanotechnology},
year={2016},
month={Jan},
day={01},
volume={11},
number={1},
pages={37-41},
abstract={Single-photon emission at room temperature can be achieved with hexagonal boron nitride due to electron and hole confinement in vacancy-related defects.},
issn={1748-3395},
doi={10.1038/nnano.2015.242},
url={https://doi.org/10.1038/nnano.2015.242}
}

@article{Sajid,
doi = {10.1088/1361-6633/ab6310},
url = {https://dx.doi.org/10.1088/1361-6633/ab6310},
year = {2020},
month = {mar},
publisher = {IOP Publishing},
volume = {83},
number = {4},
pages = {044501},
author = {A Sajid and Michael J Ford and Jeffrey R Reimers},
title = {Single-photon emitters in hexagonal boron nitride: a review of progress},
journal = {Reports on Progress in Physics}

}


@article{ziegler1977calculation,
  title={On the calculation of multiplet energies by the Hartree-Fock-Slater method},
  author={Ziegler, Tom and Rauk, Arvi and Baerends, Evert J},
  journal={Theoretica chimica acta},
  volume={43},
  pages={261--271},
  year={1977},
  publisher={Springer}
}

@article{vonBarth1979,
  title = {Local-density theory of multiplet structure},
  author = {von Barth, Ulf},
  journal = {Phys. Rev. A},
  volume = {20},
  issue = {4},
  pages = {1693--1703},
  numpages = {0},
  year = {1979},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.20.1693},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.20.1693}
}

@article{Paszkowicz,
author={Paszkowicz, W.
and Pelka, J. B.
and Knapp, M.
and Szyszko, T.
and Podsiadlo, S.},
title={Lattice parameters and anisotropic thermal expansion of hexagonal boron nitride in the 10--297.5 K temperature range},
journal={Applied Physics A},
year={2002},
month={Sep},
day={01},
volume={75},
number={3},
pages={431-435},
issn={1432-0630},
doi={10.1007/s003390100999},
url={https://doi.org/10.1007/s003390100999}
}

@Article{Huang1950,
author={Huang, Kun and Rhys, Avril},
title={Theory of light absorption and non-radiative transitions in {F}-centres},
journal={Proc. R. Soc. Lond. Series A},
year={1950},
month={Dec},
day={22},
publisher={Royal Society},
volume={204},
number={1078},
pages={406-423},
doi={10.1098/rspa.1950.0184},
url={https://doi.org/10.1098/rspa.1950.0184}
}

@article{Udvarhelyi,
  title = {Spectrally Stable Defect Qubits with no Inversion Symmetry for Robust Spin-To-Photon Interface},
  author = {Udvarhelyi, P\'eter and Nagy, Roland and Kaiser, Florian and Lee, Sang-Yun and Wrachtrup, J\"org and Gali, Adam},
  journal = {Phys. Rev. Appl.},
  volume = {11},
  issue = {4},
  pages = {044022},
  numpages = {8},
  year = {2019},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevApplied.11.044022},
  url = {https://link.aps.org/doi/10.1103/PhysRevApplied.11.044022}
}

